EfficientPhys: Enabling Simple, Fast and Accurate Camera-Based Vitals Measurement

Camera-based physiological measurement is a growing field with neural models providing state-the-art-performance. Prior research have explored various "end-to-end" models; however these methods still require several preprocessing steps. These additional operations are often non-trivial to implement making replication and deployment difficult and can even have a higher computational budget than the "core" network itself. In this paper, we propose two novel and efficient neural models for camera-based physiological measurement called EfficientPhys that remove the need for face detection, segmentation, normalization, color space transformation or any other preprocessing steps. Using an input of raw video frames, our models achieve strong performance on three public datasets. We show that this is the case whether using a transformer or convolutional backbone. We further evaluate the latency of the proposed networks and show that our most light weight network also achieves a 33% improvement in efficiency.

==> sections/removed.tex <==
\begin{table*}[t!]
    \small
	\caption{Cross-dataset heart rate evaluation on three public datasets: UBFC, MMSE and PURE (beats per minute)}
	\vspace{0.3cm}
	\label{tab:cross_eval_crop}
	\centering
	\small
	\setlength\tabcolsep{3pt} % default value: 6pt
	\begin{tabular}{r|ccc|ccc|ccc}
	\toprule
	    &\multicolumn{3}{c}{\textbf{UBFC}} & \multicolumn{3}{c}{\textbf{PURE}} & \multicolumn{3}{c}{\textbf{MMSE}} \\
        \textbf{Method} & MAE$\downarrow$ &  RMSE$\downarrow$ & $\rho$ $\uparrow$ & MAE$\downarrow$ & RMSE$\downarrow$ & $\rho$ $\uparrow$ & MAE$\downarrow$ &  RMSE$\downarrow$ & $\rho$ $\uparrow$ \\ \hline  \hline 
        EfficientPhys-C & \textbf{1.14} & \textbf{1.81} & \textbf{0.99} & \textbf{1.33} & \textbf{5.99} & \textbf{0.97} & \textbf{2.91} & \textbf{5.43} & \textbf{0.92}  \\
        EfficientPhys-T1 & 1.53 & 2.27 & 0.99 & 2.15 & 7.98 & 0.94 & 3.48 & 7.21 & 0.86  \\
        EfficientPhys-T2 & 3.07 & 4.78 & 0.96 & 7.71 & 9.95 & 0.85 & 3.51 & 6.98 & 0.88 \\ \hdashline
        TS-CAN\cite{liu_multi-task_2020}& 1.70 & 2.72 & 0.99 & 2.48 & 9.01 & 0.92 & 3.85 & 7.21 & 0.86  \\
        POS\cite{wang_algorithmic_2017} & 3.52 & 8.38 & 0.90 & 3.14 & 10.57 & 0.95 & 3.98 & 6.66 & 0.67\\
        CHROM\cite{de2013robust} & 3.10 & 6.84 & 0.93 & 2.07 & 9.92 & \textbf{0.99} & 7.31 & 9.85 & 0.57 \\
        ICA\cite{poh2010advancements}& 4.39 & 11.60 & 0.82 & 5.70 & 18.10 & 0.70 & 10.2 & 14.4 & 0.50 \\
       \bottomrule 
       \end{tabular}
       \\
       \tiny
      MAE = Mean Absolute Error in HR estimation, RMSE = Root Mean Square Error in HR estimation, $\rho$ = Pearson Correlation in HR estimation.
    \vspace{-0.1cm}
\end{table*}
